Modeling Ringdown: Beyond the Fundamental Quasi-Normal Modes

While black hole perturbation theory predicts a rich quasi-normal mode structure, technical challenges have limited the numerical study of excitations to the fundamental, lowest order modes caused by the coalescence of black holes. Here, we present a robust method to identify quasi-normal mode excitations beyond the fundamentals within currently available numerical relativity waveforms. In applying this method to waveforms of initially non-spinning black hole binaries, of mass ratios 1 to 15, we find not only the fundamental quasi-normal mode amplitudes, but also overtones, and evidence for 2nd order quasi-normal modes. We find that the mass-ratio dependence of quasi-normal mode excitation is very well modeled by a Post-Newtonian like sum in symmetric mass ratio. Concurrently, we find that the mass ratio dependence of some quasi-normal modes is qualitatively different from their Post-Newtonian inspired counterparts, suggesting that the imprints of nonlinear merger are more evident in some modes than in others. We present new fitting formulas for the related quasi-normal mode excitations, as well as for remnant black hole spin and mass. We also discuss the relevance of our results in terms of gravitational wave detection and characterization.

==> ang_coeffs_table.tex <==
\begin{tabular}{|c|| p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} |} 
	\hline 
	\hline 
	$(l,m,n)$ & $\alpha_0$ & $\alpha_1$ & $\alpha_2$ & $\alpha_3$ & $\alpha_4$ \\ 
	\hline 
	\hline 
	$(2,1,0)$ & $2.417$ & $-2.647$ & $-2.042$ & $0$ & $0$\\ 
	\hline 
	$(2,2,0)$ & $0.05992$ & $-2.208$ & $0.2412$ & $0$ & $0$\\ 
	\hline 
	$(2,2,1)$ & $-2.936$ & $0.129$ & $2.961$ & $0$ & $0$\\ 
	\hline 
	$(2,2,2)$ & $0.2528$ & $-2.928$ & $0.08554$ & $0$ & $0$\\ 
	\hline 
	$(3,2,0)$ & $-0.7712$ & $1.71$ & $-2.036$ & $-2.553$ & $0$\\ 
	\hline 
	$(3,3,0)$ & $-0.1153$ & $1.528$ & $-1.131$ & $1.747$ & $0$\\ 
	\hline 
	$(3,3,1)$ & $-2.726$ & $0.3594$ & $-2.938$ & $-1.683$ & $0$\\ 
	\hline 
	$(4,3,0)$ & $2.285$ & $-1.541$ & $1.39$ & $-1.077$ & $1.897$\\ 
	\hline 
	$(4,4,0)$ & $0.008012$ & $2.588$ & $-0.4417$ & $2.729$ & $-0.5777$\\ 
	\hline 
	$(5,4,0)$ & $2.077$ & $-2.134$ & $0.1512$ & $2.731$ & $-0.8791$\\ 
	\hline 
	$(5,5,0)$ & $3.123$ & $-0.5147$ & $2.841$ & $-0.1611$ & $2.886$\\ 
	\hline 
	\hline 
\end{tabular} 


==> fit_coeffs_table.tex <==
\begin{tabular}{|c|| p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} |} 
	\hline 
	\hline 
	$(l,m,n)$ & $c_0$ & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ \\ 
	\hline 
	\hline 
	$(2,1,0)$ & $0.04584$ & $-0.03155$ & $0.4989$ & $0$ & $0$ & $0$ & $0$\\ 
	\hline 
	$(2,2,0)$ & $0.06365$ & $-0.7321$ & $5.585$ & $0$ & $0$ & $0$ & $0$\\ 
	\hline 
	$(2,2,1)$ & $0.555$ & $-5.663$ & $18.7$ & $0$ & $0$ & $0$ & $0$\\ 
	\hline 
	$(2,2,2)$ & $0.7767$ & $-8.26$ & $23.27$ & $0$ & $0$ & $0$ & $0$\\ 
	\hline 
	$(3,2,0)$ & $0.005461$ & $-0.07637$ & $0.5894$ & $-2.725$ & $5.063$ & $0$ & $0$\\ 
	\hline 
	$(3,3,0)$ & $0.03758$ & $-1.105$ & $13.8$ & $-66.36$ & $127.7$ & $0$ & $0$\\ 
	\hline 
	$(3,3,1)$ & $0.669$ & $-18.35$ & $194.6$ & $-893.2$ & $1529$ & $0$ & $0$\\ 
	\hline 
	$(4,3,0)$ & $0.002311$ & $-0.08447$ & $1.517$ & $-14.6$ & $75.93$ & $-203.8$ & $226.8$\\ 
	\hline 
	$(4,4,0)$ & $0.003038$ & $-0.08824$ & $1.738$ & $-17.5$ & $95.92$ & $-284.7$ & $358.6$\\ 
	\hline 
	$(5,4,0)$ & $0.0003404$ & $-0.01127$ & $0.1826$ & $-1.719$ & $9.273$ & $-26.16$ & $29.71$\\ 
	\hline 
	$(5,5,0)$ & $0.001451$ & $-0.05178$ & $1.04$ & $-10.81$ & $61.29$ & $-187.2$ & $245.3$\\ 
	\hline 
	\hline 
\end{tabular} 


==> fit_phase_coeffs_table.tex <==
\begin{tabular}{|c|| p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} |} 
	\hline 
	\hline 
	$(l,m,n)$ & $d_0$ & $d_1$ & $d_2$ & $d_3$ \\ 
	\hline 
	\hline 
	$(2,1,0)$ & $2.592$ & $0.1921$ & $0.2124$ & $59.14$\\ 
	\hline 
	$(2,2,0)$ & $-68.92$ & $669.1$ & $-1141$ & $0$\\ 
	\hline 
	$(2,2,1)$ & $1.803$ & $0.07632$ & $0.212$ & $170.5$\\ 
	\hline 
	$(2,2,2)$ & $4.879$ & $0.2216$ & $0.173$ & $-374.7$\\ 
	\hline 
	$(3,2,0)$ & $3.133$ & $3.006$ & $0.2129$ & $67.39$\\ 
	\hline 
	$(3,3,0)$ & $0.4792$ & $0.4883$ & $0.2121$ & $12.97$\\ 
	\hline 
	$(3,3,1)$ & $4.668$ & $1.023$ & $0.2184$ & $24.17$\\ 
	\hline 
	$(4,3,0)$ & $0.4035$ & $2.677$ & $0.1756$ & $-389.1$\\ 
	\hline 
	$(4,4,0)$ & $4.836$ & $2.246$ & $0.2265$ & $-97.5$\\ 
	\hline 
	$(5,4,0)$ & $4.292$ & $3.121$ & $0.2353$ & $-248$\\ 
	\hline 
	$(5,5,0)$ & $5.345$ & $1.528$ & $0.1986$ & $-38.15$\\ 
	\hline 
	$(2,2,0)(2,2,0)$ & $5.997$ & $0.08591$ & $0.2036$ & $254.5$\\ 
	\hline 
	$(2,2,0)(3,3,0)$ & $1.545$ & $6.29$ & $0.4344$ & $1.404$\\ 
	\hline 
	\hline 
\end{tabular} 


==> mag_coeffs_table.tex <==
\begin{tabular}{|c|| p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} | p{\rscale cm} |} 
	\hline 
	\hline 
	$(l,m,n)$ & $|a_0|$ & $|a_1|$ & $|a_2|$ & $|a_3|$ & $|a_4|$ \\ 
	\hline 
	\hline 
	$(2,1,0)$ & $0.2045$ & $0.3554$ & $1.034$ & $0$ & $0$\\ 
	\hline 
	$(2,2,0)$ & $0.184$ & $0.1$ & $5.088$ & $0$ & $0$\\ 
	\hline 
	$(2,2,1)$ & $0.8904$ & $6.304$ & $19.4$ & $0$ & $0$\\ 
	\hline 
	$(2,2,2)$ & $1.626$ & $15.3$ & $40.65$ & $0$ & $0$\\ 
	\hline 
	$(3,2,0)$ & $0.06907$ & $0.4579$ & $0.7754$ & $2.476$ & $0$\\ 
	\hline 
	$(3,3,0)$ & $0.07896$ & $0.9093$ & $5.345$ & $20.66$ & $0$\\ 
	\hline 
	$(3,3,1)$ & $0.7784$ & $7.641$ & $25.73$ & $10.29$ & $0$\\ 
	\hline 
	$(4,3,0)$ & $0.03099$ & $0.3174$ & $1.544$ & $6.013$ & $16.33$\\ 
	\hline 
	$(4,4,0)$ & $0.05596$ & $0.7825$ & $7.74$ & $41.32$ & $82.02$\\ 
	\hline 
	$(5,4,0)$ & $0.01222$ & $0.1674$ & $1.834$ & $8.804$ & $16.32$\\ 
	\hline 
	$(5,5,0)$ & $0.03257$ & $0.4652$ & $4.876$ & $28.71$ & $64.31$\\ 
	\hline 
	\hline 
\end{tabular} 

